Dark matter axion detection in the radio/mm-waveband

We discuss axion dark matter detection via two mechanisms: spontaneous decays and resonant conversion in neutron star magnetospheres. For decays, we show that the brightness temperature signal, rather than flux, is a less ambiguous measure for selecting candidate objects. This is owing principally to the finite beam width of telescopes which prevents one from being sensitive to the total flux from the object. With this in mind, we argue that the large surface-mass-density of the galactic centre or the Virgo cluster centre offers the best chance of improving current constraints on the axion-photon coupling via spontaneous decays. For the neutron star case, we first carry out a detailed study of mixing in magnetised plasmas. We derive transport equations for the axion-photon system via a controlled gradient expansion, allowing us to address inhomogeneous mass-shell constraints for arbitrary momenta. We then derive a non-perturbative Landau-Zener formula for the conversion probability valid across the range of relativistic and non-relativistic axions and show that the standard perturbative resonant conversion amplitude is a truncation of this result in the non-adiabatic limit. Our treatment reveals that that infalling dark matter axions typically convert non-adiabatically in magnetospheres. We describe the limitations of one-dimensional mixing equations and explain how three-dimensional effects activate new photon polarisations, including longitudinal modes and illustrate these arguments with numerical simulations in higher dimensions. We find that the bandwidth of the radio signal is dominated by Doppler broadening from the relative motion of the neutron star with respect to the observer. Therefore, we conclude that the radio signal from the resonant decay is weaker than previously thought, which means one relies on local density peaks to probe weaker axion-photon couplings.

==> Sec_C_Optimizing_Target_Objects.tex <==
\subsection{Optimising Target Objects}\label{subsec:SpontTarget}

\begin{figure*}[!t]
 \centering
 \includegraphics[width=0.45\textwidth]{Scatter_Plot1.pdf}
 \includegraphics[width=0.45\textwidth]{Scatter_Plot2.pdf} \\
 %\includegraphics[width=0.45\textwidth]{testplot1.pdf}
 %\includegraphics[width=0.45\textwidth]{testplot2.pdf}
 \caption{In the {\em left} panel. Signal strength as given by $\Sigma/\Delta v \propto T_{RJ}$. We assume an \textit{identical} object and beam size  $\Sigma = M_{\rm obj}/(\theta_{\rm obj} D_{\rm obj})^2$ taking values from table~\ref{ClusterCalculations}. Note we normalised $\Sigma$ by the background value $1.2\times 10^{-9}\,{\rm kg}\,{\rm m}^{-3}\,{\rm s}$ for the data in table appears relatively flat - the solid green line - and is compatible with the simple argument presented in the text, albeit with a somewhat higher value ($\approx 500$) relative to the background value. Possibly there is a trend with mass which we denoted with a line $\propto M^{-0.2}$ which could be due to the concentration parameter varying as a function of mass and the fact that the angular sizes are probably the scale radius for some fitted profile function rather than the virial radius. We note that much of this trend is driven by the outliers at low mass, ultra-faint dwarf spheroidal, and high mass, the galaxy clusters, VIRGO and COMA. As with the bottom panel we present results using both $\Delta v_{\rm obj}$ and $\Delta v_{\rm int}$ which are broadly consistent. In the {\em right} panel, we present the quantity in \eqref{eqn:CaputoQuantity} for the data in table~\ref{ClusterCalculations} which clearly increases like $\theta_{\rm obj}^2$ as denoted by the line in the plot. Note that the starred data points, which use observational measurements of the velocity width $\Delta v_{\rm obj}$, and the circular points, which correspond to the inferred width $\Delta v_{\rm inf} \approx \left(GM_{\rm obj}/R_{\rm obj}\right)^{1/2}$, show the same trend. }
 \label{fig:ScatterPlots}
\end{figure*}

In the previous two sections we have explained that, if one targets a halo with surface mass density $\Sigma_{\rm beam}\approx 0.07\,{\rm kg}\,{\rm m}^{-2}$ and velocity width $\Delta v\approx 200\,{\rm Km}\,{\rm s}^{-1}$, the signal from spontaneous decay combined with stimulated emission from the CMB for $g_{\rm a\gamma\gamma}=10^{-10}\,{\rm GeV}^{-1}$ is too weak to be detected even for an array of receivers with $N\lesssim 10^{6}$. We came to this conclusion by estimating the integration time required to detect the signal focusing on the expression for the signal expressed in terms of the brightness temperature (\ref{ref:brighttemp_again}).



Examination of this equation makes it clear that the largest possible signal is obtained by maximising $\Sigma_{\rm beam}/\Delta v$. If the object is such that $\theta_{\rm FHWM}\approx \theta_{\rm vir}$, we estimate the quantity to be $\approx 3.5\times 10^{-7}\,{\rm kg}\,{\rm m}^{-3}\,{\rm s}^{-1}$ for the strawman object used in the previous section which is around 300 times larger than the background value. This value is based on what we think, at a level of better than a factor two, are realistic values, but precise knowledge of it is absolutely critical to any attempt to improve the CAST limits of $g_{\rm a\gamma\gamma}$ using this approach. In this section, we will discuss, using theoretical arguments and comparing to observations, the range of values for $\Sigma_{\rm beam}/\Delta v$ that might be available for us to be observed in the Universe.

One might wonder how $\Sigma_{\rm vir}/\Delta v$ depends on the size of the object. If we consider a halo with virial overdensity $\Delta_{\rm vir}\sim 100$, then $M_{\rm vir}=\tfrac{4\pi}{3}\Delta_{\rm vir}\rho_{\rm a} R_{\rm vir}^3$, where $\rho_{\rm a}=\Omega_{\rm a}\rho_{\rm crit}$ is the background density of axions and $\rho_{\rm crit}$ is the critical density. An estimate for the velocity width, up to order one factors, is $\Delta v=(GM_{\rm vir}/R_{\rm vir})^{1/2}$ and hence we find that 
\begin{equation}\label{eqn:SigmaQuantity}
\frac{\Sigma_{\rm vir}}{\Delta v}\approx 0.7\left(\frac{\Delta_{\rm vir}\rho_{\rm a}}{G}\right)^{1/2}\approx 3.5\times 10^{-7}\,{\rm kg}\,{\rm m}^{-3}\,{\rm s}\,,
\end{equation}
which is independent of the size of the object - that is, there is no dependence on $M_{\rm vir}$ or $R_{\rm vir}$. If $\Delta_{\rm vir}$ is universal and independent of the size of the object, as it is supposed to be almost by definition, then the expected brightness temperature averaged over a virialised halo will be independent of the size and hence the optimal detection for a specific halo size and telescope configuration would be obtained by matching the size of the object approximately to the telescope beam width. This is the standard practice to optimise detection efficiency in all branches of astronomy.

This suggestion that there is no optimal size of object appears to be contrary to the conclusions of \cite{ref:Caputo,ref:Caputo1}, who claimed that the optimal detection would be for dwarf spheroidal galaxies, that is the very lowest mass halos. They came to this conclusion considering the quantity 
\begin{equation}\label{eqn:CaputoQuantity}
 \frac{1}{\Delta v}\int \mathrm{d}\Omega \mathrm{d}l\rho_{\rm a}\propto \frac{M_{\rm beam}}{d^2\Delta v}\propto S_{\rm beam}\,,
\end{equation}
where $d$ is the distance to the object and the angular integration over the angular size of the object - or, as they state it, for a telescope beam which has the same size as the object. This quantity is $\propto S_{\rm beam}$ defined in \eqref{eqn:FluxValue} which is equivalent to (\ref{ref:brighttemp}) if one is careful with the choice of $\Sigma_{\rm beam}$. But we have already explained that one can come to the wrong conclusion if one uses the wrong value of $M_{\rm beam}$ for a specific halo and that it is actually better to think in terms of the surface mass density $\Sigma_{\rm beam}$. If one were to integrate out to the size of the object $S_{\rm beam}=S_{\rm tot}$, one would expect this to be $\propto\theta_{\rm FWHM}^2$ as they find.

In fig.~\ref{fig:ScatterPlots}, we have plotted the quantities in \eqref{eqn:CaputoQuantity} and \eqref{eqn:SigmaQuantity} using the data in table~\ref{ClusterCalculations} which is similar to, but not exactly the same as, that used in \cite{ref:Caputo,ref:Caputo1}. In particular we have added some galaxies and galaxy clusters to the dwarf galaxies which they focus on that enables us to probe a wider lever arm in mass. The table contains values for the distance to and the mass of the object $D_{\rm obs}$ and $M_{\rm obj}$, respectively, the angular size $\theta_{\rm obj}$ and the velocity width $\Delta v_{\rm obj}$. These are inferred in a heterogeneous way, but should at least be indicative of some truth. We would not necessarily expect these values to be those for a virialised halo and therefore we denoted them with the suffix ``obj" to distinguish them as being observationally determined. From the observed information, we can infer the radius, $R_{\rm obj}=\theta_{\rm obj}/(2D_{\rm obj}$ and also check consistency with our analytic estimates above by inferring $\Delta v_{\inf}=(GM_{\rm obj}/R_{\rm obj})^{1/2}$, as well as calculating the surface mass density appropriate to an average over the object radius, $\Sigma_{\rm obj}=M_{\rm obj}/(\pi R_{\rm obj}^2)$.

Firstly, we find in the right panel of fig.~\ref{fig:ScatterPlots} that \eqref{eqn:CaputoQuantity} which was plotted in \cite{ref:Caputo1} is indeed $\propto\theta_{\rm obj}^2$ as claimed. But on the basis of the theoretical argument above, this is exactly what one would expect for the total flux density $S_{\rm tot}\propto \Sigma_{\rm ave}\theta^2/\Delta v$, where $\Sigma_{\rm ave}$ is some average surface mass density for the objects, and hence, while it provides some confidence that the modelling is correct, it does not yield any obvious information about which objects would be optimal.

In the left panel of fig.~\ref{fig:ScatterPlots} we have plotted $\Sigma_{\rm obj}/\Delta v$ for the data presented in table~\ref{ClusterCalculations}, using both $\Delta v_{\rm obj}$ and $\Delta v_{\inf}$ with consistent results. We find that the data are compatible with $\Sigma_{\rm beam}/\Delta v$ being a constant over eight orders of magnitude and for it to be $\approx 500$ times the background value - slightly higher than for our strawman object - within the kind of uncertainties that we might expect coming from a heterogeneous sample such as the one which we have used. Visually, there could be some evidence for a trend $\sim M^{-0.2}$ which we have also included to guide the eye, but the evidence for this is largely due to a few outliers at the low- and high-mass ends where perhaps the observational estimate are most uncertain. So it could be that there is some preference for lower mass halos over high mass halos, but the effect is not very dramatic. Note that on the $y-$axis, we plot $\left(\Sigma/\Delta v\right)^{\rm rel} \equiv \frac{\Sigma/\Delta v}{1.2\times 10^{-9}\,{\rm kg\,m^{-3}\,s}}$, where the denominator is the value associated to the background.

It could be that the possible trend seen in the left panel of fig.~\ref{fig:ScatterPlots} is related to the concentration parameter of the halo. It is likely that the observationally determined angular size, $\theta_{\rm obj}$, is not the virial radius but some scale radius from a fitting function used in conjunction with images. If this is the case, then we might expect a weak trend with mass.

The concentration parameter has been computed in numerical simulations and is usually assumed to be universal for halos of a given mass, $M$. A recently proposed expression is~\cite{ref:MultiDark}
\begin{equation}
 {\hat c}(M,z)={\hat c}_0(z)\left(\frac{M}{ M_0}\right)^{-\gamma(z)}\left[1+\left(\frac{M}{M_1(z)}\right)^{0.4}\right]\,,
\end{equation}
where $M_0=10^{12}h_{100}^{-1}M_{\odot}$ and $\hat{c}_0(z)$, $\gamma(z)$ and $M_1(z)$ are fitted parameters which are redshift dependent. We will focus on low redshifts where $\hat{c}_0(z)\approx 7.4$, $\gamma(0)\approx 0.12$ and $M_1(0)=5.5\times 10^{17}h_{100}^{-1}M_{\odot}$. 
From this we see that at $z=0$, $\hat{c}\propto M^{-0.12}$, that is, lower mass halos typically are more concentrated than higher mass halos, and therefore there will be more mass inside the scale radius, and for observations focussing on the region inside this scale radius $\Sigma_{\rm beam}$ might be larger.

\begin{table*}
 \centering
 \begin{tabular}{|l|c|c|c|c|c|}
 \hline
 Object  & $D_{\rm obj}$ & $M_{\rm obj}$ ($\rm M_{\odot}$) & $\theta_{\rm obj}$ & $\Delta v_{\rm obj}$ [$\rm km\,s^{-1}$] & Reference(s)  \\
 \hline
 Leo 1 &  $250\pm 30$  kpc & $2.2\times 10^{7}$ & $12.6\pm1.5$ arcmin & 8.8 & \cite{ref:Mateo} \\
 NGC 6822 &  $490\pm 40$ kpc & $1.6\times 10^9$ & $40\pm 10$ arcmin & 8 & \cite{ref:Mateo} \\
 Draco &  $82\pm 6$ kpc & $2.2\times10^{7}$ & $28.3\pm 2.4$ arcmin & 9.5 & \cite{ref:Mateo} \\
 Wilman 1 & 45 kpc & $4\times 10^5$ & 9 arcmin & 4 & \cite{ref:DwarfGalMass}  \\
 Reticulum 2 &  30 kpc & $5.6 \pm 2.4\times 10^5$ & $3.64^{+0.21}_{-0.12}$ arcmin & 3.3 &\cite{ref:Beasts, ref:Reticulum2} \\
 Sextans B & 1345 kpc& $3.95\times 10^8$ & 3.9 arcmin & 18 & \cite{ref:Mateo}\\ 
 Pegasus & 955 kpc& $5.8 \times 10^{7}$ & 3.9 arcmin & 8.6 & \cite{ref:Mateo} \\
 Antlia & 1235 kpc& $1.2\times 10^7$ & 5.2 arcmin & 6.3 & \cite{ref:Mateo} \\
 NGC 205 & 815 kpc& $7.4\times 10^{8}$ & 6.2 arcmin& 16 & \cite{ref:Mateo}\\
 \hline
 NGC 5128 & 3.75 Mpc & $5.07\times 10^{11}$ & 34.67 arcmin & 477 & \cite{ref:NearGalCat} \\
 NGC 5194 & 15.85 Mpc & $4.17\times 10^{10}$ & 8.4 arcmin & 175 & \cite{ref:NearGalCat} \\
 Maffei2 & 2.8 Mpc & $4.17\times 10^{10}$ & 3.8 arcmin & 306 & \cite{ref:NearGalCat} \\
 IC2574 & 4.02 Mpc &  $4.57\times 10^9$ & 13.18 arcmin & 107 & \cite{ref:NearGalCat} \\
 SexA & 1.32 Mpc & $2.51\times 10^8$ & 5.89 arcmin & 46 & \cite{ref:NearGalCat} \\
 NGC 3556 & 9.9 Mpc & $3.31\times 10^{10}$ & 5.01 arcmin & 308 & \cite{ref:NearGalCat} \\
 IC 0342 & 3.28 Mpc & $1.41\times 10^{11}$ & 21.38 arcmin & 181 & \cite{ref:NearGalCat} \\
 NGC 6744 & 8.3 Mpc & $2.24\times 10^{11}$ & 21.38 arcmin & 323 &\cite{ref:NearGalCat}\\
 ESO 300-014 & 9.8 Mpc & $10^{10}$ & 7.08 arcmin & 130 & \cite{ref:NearGalCat}\\
 NGC 3184 & 11.12 Mpc & $6.3\times 10^{10}$ & 7.41 arcmin & 128 & \cite{ref:NearGalCat}\\
 \hline
 Virgo & $18 \pm 1.2$ Mpc & 2.91$\times 10^{15}$ &  7 degrees & 1100 & \cite{ref:VirgoMass1,ref:VirgoMass2}  \\
 Coma & 100 Mpc & 3$\times 10^{15}$ & 100 arcmin & 1100 & \cite{ref:ComaMass, ref:ComaDistance}\\
 \hline
 \end{tabular}
 \caption{Table of masses ($M_{\rm obj}$), distances ($D_{\rm obj}$), angular sizes ($\theta_{\rm obj})$ and velocity widths ($\Delta v_{\rm obj})$ extracted from the literature and used in fig.~\ref{fig:ScatterPlots}. In each case we have specified the reference of the paper from which the numbers are calculated. From paper to paper the methods employed are very different and hence the overall sample is relatively heterogeneous. For each object we can infer a radius $R_{\rm obj}=\theta_{\rm obj}D_{\rm obj}/2$ and a velocity width $\Delta v_{\rm inf}=(GM_{\rm obj}/R_{\rm obj})^{1/2}$. We find that $\Delta v_{\rm obj}$ is strongly correlated with $\Delta v_{\rm inf}$ as we would expect and indeed that $M_{\rm obj}$ is also correlated with $R_{\rm obj}$.}
\label{ClusterCalculations}
\end{table*}

\begin{figure}[t]
 \centering
 \includegraphics[width = 0.45\textwidth,height=0.45\textwidth]{G_Func.pdf}
 \caption{The function $G(\hat{c}, \tilde{R})$ as a function of its arguments. In the left panel, we plot $G$ as a function of $\hat{c}$ for different values constant $\tilde{R}$, and vice versa in the right panel. }
 \label{fig:GFunction}
\end{figure}

This leads us on to an important caveat in this discussion: one does not have to choose to focus on trying to detect the entire signal from a halo and indeed it will be optimal, as well as practical, to not do this. Using (\ref{ref:mbeam}) we can deduce that 
\begin{equation}
 \Sigma_{\rm beam}=G\left(\hat{c},{\frac{R_{\rm beam}}{R_{\rm vir}}}\right)\Sigma_{\rm vir}\,,
\end{equation}
for an NFW profile where $G(x,y)=x^2\log(2y/x)/f(x)$ for $y/x\ll 1$. We anticipate that one could derive a similar expression for any halo profile. We plot the function $G(\hat{c}, \frac{R_{\rm beam}}{R_{\rm vir}})$ as a function of $\hat{c}$ and $\tilde{R} = R_{\rm beam}/R_{\rm vir}$, in fig.~(\ref{fig:GFunction}) which indicates that enhancements of up to 100 might easily be possible and that these are likely to be larger in lower mass objects than those of higher mass. Therefore, it is clear that, for a fixed experimental set up ($R_{\rm vir}/R_{\rm beam}$ fixed), one should search for an object with the largest concentration, a general result which we already anticipated in section~\ref{subsec:SpontSignal}.

In conclusion, we have argued that maximizing $\Sigma_{\rm beam}/\Delta v$ will give the largest possible brightness temperature signal. Theoretical arguments suggest that if the beam encloses the virial radius of a particular object, this will be independent of mass and a very rudimentary search of the literature for specific values suggests that this could be true. However, for fixed observational setup, and hence fixed resolution, one might find a significant enhancement of the signal due to the fact that the surface mass density will increase as one probes the more central regions of a halo. These are likely to be larger for smaller mass objects since they are on average more concentrated. This is the reason we have presented our sensitivity estimates as a function of $\Sigma_{\rm beam}$ and results for range of values $\Sigma_{\rm beam}=0.07-0.7\,{\rm kg}\,{\rm m}^{-2}$ in fig.~\ref{fig:CMB_Enhancement}. 

